Wireless Edge Content Broadcast via Integrated Terrestrial and Non-terrestrial Networks

Non-terrestrial networks (NTN) have emerged as a transformative solution to bridge the digital divide and deliver essential services to remote and underserved areas. In this context, low Earth orbit (LEO) satellite constellations offer remarkable potential for efficient cache content broadcast in remote regions, thereby extending the reach of digital services. In this paper, we introduce a novel approach to optimize wireless edge content placement using NTN. Despite wide coverage, the varying NTN transmission capabilities must be carefully aligned with each content placement to maximize broadcast efficiency. In this paper, we introduce a novel approach to optimize wireless edge content placement using NTN, positioning NTN as a complement to TN for achieving optimal content broadcasting. Specifically, we dynamically select content for placement via NTN links. This selection is based on popularity and suitability for delivery through NTN, while considering the orbital motion of LEO satellites. Our system-level case studies, based on a practical LEO constellation, demonstrate the significant improvement in placement speed compared to existing methods, which neglect network mobility. We also demonstrate that NTN links significantly outperform standalone wireless TN solutions, particularly in the early stages of content delivery. This advantage is amplified when there is a higher correlation of content popularity across geographical regions.

==> 07_Acknowledgments.tex <==
\section{Acknowledgments}

F.~Wang and T.~Q.~S.~Quek were supported in part by the National Research Foundation, Singapore and Infocomm Media Development Authority under its Future Communications R\&D Programme. 
G.~Geraci was supported in part by the Spanish Research Agency through grants PID2021-123999OB-I00 and CEX2021-001195-M, by the UPF-Fractus Chair, and by the Spanish Ministry of Economic Affairs and Digital Transformation and the European Union NextGenerationEU through the UNICO 5G I+D SORUS project.

==> 0X_TableParameters_NTN.tex <==
\begin{table}[!t]
\renewcommand{\arraystretch}{1.3} 
\caption{Main NTN system-level parameters\label{tab:tableparametersNTN}. }
\centering
\setlength{\tabcolsep}{2mm}{
\begin{tabular}{c|c}

\toprule
\textbf{Parameter} & \textbf{Value} \\ 
\hline 
LEO orbital altitude \cite{SpaceX} & 550\,km \\ \hline 
Minimum elevation angle & 10$\mathrm{{}^\circ}$ \\ \hline 
Number of LEO satellites & 1584 \\ \hline 
Satellite inclination & 53$\mathrm{{}^\circ}$ \\ \hline 
Satellite antenna pattern \cite{3GPP38821} & Reflector antenna with circular aperture \\ \hline 
Satellite beam diameter & 20\,km \\ \hline 
Satellite transmit power \cite{3GPP38811} & 30\,dBW \\ \hline 
Transmit antenna gain & 38.5\,dBi \\ \hline 
Receive antenna gain  & 39.7\,dBi \\ \hline 
Link bandwidth & 100\,MHz \\ \hline 
\bottomrule
\end{tabular}}
\end{table}

==> 0X_TableParamters_ContentPopularity.tex <==
\begin{table}[!t]
\renewcommand{\arraystretch}{1.3} 
\caption{Main Cache Content Popularity parameters\label{tab:tableparametersContentPopularity}}
\centering
\setlength{\tabcolsep}{2mm}{
\begin{tabular}{c|c}

\toprule
\textbf{Parameter} & \textbf{Value} \\ \hline 
Content popularity distribution & Zipf distribution \\ \hline 
Number of files cached by TN BS & 50 \\ \hline 
Cache file size & 20 MB \\ \hline 
Cache content skewness & $\alpha_{r}=1$ \\ \hline 
Regional file correlation & $\rho=0.8$ \\ \hline 
\bottomrule
\end{tabular}}
\end{table}

==> 0X_TableParamters_TN.tex <==
\begin{table}[!t]
\renewcommand{\arraystretch}{1.3} 
\caption{Main TN system-level parameters\label{tab:tableparametersTN}.}
\centering
\setlength{\tabcolsep}{2mm}{
\begin{tabular}{c|c}

\toprule
\textbf{Parameter} & \textbf{Value} \\ \hline 
Geographical area served & [33-39$\mathrm{{}^\circ}$N], [87-93$\mathrm{{}^\circ}$E] \\ \hline 
Number of geographical regions & 6 \\ \hline 
Size of each region & 1200\,km${}^{2}$ \\ \hline 
Total number of BSs & 600 \\ \hline 
BS coverage radius \cite{DowFraSha2020} & 2\,km \\ \hline 
BS transmit power \cite{3GPP38901} & 44\,dBm \\ \hline 
Transmit and receive antenna gain & 16\,dBi \\ \hline 
Link bandwidth & 100\,MHz \\ \hline
\bottomrule
\end{tabular}}
\end{table}
